Kernel Stein Discrepancy on Lie Groups: Theory and Applications

Distributional approximation is a fundamental problem in machine learning with numerous applications across all fields of science and engineering and beyond. The key challenge in most approximation methods is the need to tackle the intractable normalization constant pertaining to the parametrized distributions used to model the data. In this paper, we present a novel Stein operator on Lie groups leading to a kernel Stein discrepancy (KSD) which is a normalization-free loss function. We present several theoretical results characterizing the properties of this new KSD on Lie groups and its minimizers namely, the minimum KSD estimator (MKSDE). Proof of several properties of MKSDE are presented, including strong consistency, CLT and a closed form of the MKSDE for the von Mises-Fisher distribution on SO(N). Finally, we present experimental evidence depicting advantages of minimizing KSD over maximum likelihood estimation.

==> Rebuttals/FirstRebuttal.tex <==


\author{Xiaoda Qu, Xiran Fan, Baba C. Vemuri \thanks{Manuscript received February 2024}}

\begin{center}
{\Large \bf Kernel Stein Discrepancy on Lie Groups: Theory and Applications}
\end{center}

\begin{center}
{\large Xiaoda Qu, Xiran Fan, Baba C. Vemuri}
\end{center}
\vspace{5mm}

\section*{\bf\large Response to Reviewers}

\setcounter{page}{1}
\setcounter{subsection}{0}

We thank all the reviewers for their valuable comments and value all the reviewers' suggestions for improving the clarity and organization of our work. We have addressed each key question and concern raised by the reviewers in the following paragraphs. We hope you find our responses and revision satisfactory. The citations used in this response to reviewers are in the bibliography of the revised submission.

\subsection{\bf Response to Reviewer-1}

\subsubsection{\bf On Comparison to Barp's work}

We will first focus on the key issue raised by the reviewer namely, one of, not using large kernels, e.g., Sobolev-type kernels in our work presented here. We would like to clarify a fact first: Suppose $M$ is a manifold embedded in the Euclidean space $\mathbb{R}^d$, $k$ is a Sobolev-type kernel on $\mathbb{R}^d$ and $k|_{M}$ is the restriction of $k$ onto $M$. Then $k|_{M}$ is indeed a \emph{kernel on $M$ but not a Sobolev-type kernel on $M$ }, i.e., it does not necessarily generate a Sobolev space $W^s_2(M)$ of $M$.

For example, recall that the kernel function for Sobolev space $W^1_1(\mathbb{R})$ on $\mathbb{R}$ is 
\[
K_{1,1}(x,t)=\frac{1}{2} e^{-|x-t|}, \text{ for all } x,t\in\mathbb{R},
\]
see for example \cite{de2021reproducing}.
Then, we consider the embedded manifold $(0,+\infty)$ of $\mathbb{R}$, endowed with any Riemannian metric that will make $(0,+\infty)$ complete. Note that the Sobolev space $W^1_1(0,+\infty)$ is a subspace of $C_0(0,+\infty)$, i.e., every function $f\in W^1_2(0,+\infty) $ vanishes at infinity of $(0,+\infty)$, which implies $\lim_{x\to 0^+} f(x)=0$. However, the RKHS on $(0,+\infty)$ generated by  $K_{1,1}|_{(0,+\infty)}$ is obviously not a subspace of $C_0(0,+\infty)$, since the feature map itself
\[
\lim_{t\to 0^+} K_{1,1,x}(t)=\lim_{t\to 0^+} \frac{1}{2} e^{-|x-t|}=\frac{1}{2} e^{-|x|}\neq 0.
\]


In fact, \cite[Thm. 8]{de2021reproducing} proved that the Sobolev space $W^s_2(M)$, $s>\dim M/2$ of a complete, connected Riemannian manifold $M$ with bounded geometry, is an RKHS, thus the corresponding kernel function $k_s$ does exist. However, the calculation of the exact form of $k_s$ is highly complicated and dependent on the geometry of the underlying manifold $M$. 

Unfortunately, application of the KSD in practice requires the closed form of the kernel function. Until now, we only have the closed forms of the Sobolev-type kernel functions for the sphere and Euclidean space. We highly appreciate Barp's work, but their results are only applicable to the sphere and Euclidean space due to the lack of closed forms of Sobolev-type kernel functions on other manifolds.

Generally speaking, the larger the RKHS $\mathcal{H}_k$ is, the stronger properties are that the KSD $\ksd(p,q):=\sup \mathbb{E}_q[\mathcal{T}_p f]$ has. In practice, if the RKHS is too small, the KSD will not uniquely characterize $p$; if the RKHS is too large, e.g., the Sobolev space, then the closed form of the kernel function may not be available. To reach a balance, we choose the kernel in our work, which is large enough to distinguish between $p$ and other locally Lipschitz densities (but lacking in control of the weak convergence), and small enough so that it has a closed form on general manifolds.


\subsubsection{\bf On MKSDE of exponential family}

If we define the exponential family on Lie group $G$ as
\[
p(X)\propto \exp(\theta^\top\cdot \zeta(X)+\eta(X) ),\quad X\in G,
\]
then we can indeed easily derive a closed form for its MKSDE similarly to the von Mises-Fisher distribution on $\SO(N)$. We appreciate your suggestion and have included this derivation in this revision (see \S\ref{MKSDE-Exp-SO(N)}).

\subsubsection{\bf Composite kernel goodness of fit test}

Thank you for pointing out that a similar method has already been presented in \cite{key2021composite}. We will retract the claim on unconditional originality. However, we would like to point out that our method is established on Lie groups, and we do have looser/weaker conditions on the parameter space compared to their work. Note that the composite goodness of fit test using KSD in \cite{key2021composite} rests on the assumption \cite[see assumption 2]{key2021composite} that the parameter space $\Theta$ must be a compact and convex subset of $\mathbb{R}^d$. Therefore, it does not apply to cases like von Mises-Fisher distribution $p(X)\propto \exp(\tr(F^\top X))$, $F\in \mathbb{R}^{N\times N}$ where the parameter space $\mathbb{R}^{N\times N}$ is convex but not compact. 


\subsubsection{\bf Insufficient detail to reproduce the experiments
in Section V} We have now provided the code and data for reproducing the experiments via a GitHub link in the experiment section \ref{experiments}.

\subsubsection{\bf In Section V.B, comment on how these results shape up against existing KSDs on \texorpdfstring{$S^2$}{S2}. Is there any practical
advantage to the proposed construction?} 

Unfortunately, the only existing goodness of fit test using KSD that we are aware of is the work of \cite{xu2020stein} and their work is not a composite kernel goodness of fit test. Further, their work, as we pointed out in section \ref{KSDE}, assumes the existence of a global chart on the manifold, which is violated not only on the sphere but on any general Riemannian manifold. Also, they did not provide any accessible code for their algorithm.

\subsubsection{\bf Minor Comments}
 We have fixed all typos and minor inaccuracies pointed out in this revision. Reviewer suggestions and comments requiring our explicit response and explanation are addressed in what follows:
\begin{enumerate}[(a)]
\item {\it non-parametrically represented via say, a neural network$\to$ neural networks are parametric?"} 

In the ML community, some researchers consider the deep neural networks to be parameteric models and some as non-parameteric. We subscribe to the latter since
Neural networks can be thought of as non-parameteric function approximators in a somewhat similar vein to Fourier series representations of compactly supported functions, which are tagged as non-parameteric since they have a countably infinite set of coefficients. Another analogy is the Dirichlet process, also called the infinite Gaussian mixture model. Similar reasoning there as well. Informally, if a  model becomes increasingly rich as more parameters are added and if it is possible to characterize the limiting behavior then the model is non parametric. Further evidence in this regard is provided by the correspondence between infinite width neural networks and Gaussian Processes (GPs) that was first noted in Radford Neal's PhD thesis (University of Toronto), 1994. Note that GPs are considered non-parameteric models. For additional references in this context, please see Jaehoon Lee et al., ICLR 2018 and references therein. 

\item {\it "p1) the authors confuse "loss function" with "divergence"; it is
confusing to call both the negative log-likelihood and KL "loss functions"}:

In many applications, the terminology of loss function is used to indicate the quantity to be optimized (over some parameter space) for instance, divergence between distributions in a distributional approximation setting, or the likelihood function in a regression setting etc.

\item {\it "p3) "if the kernel function k is $C_0$ -universal[32], then KSD will
uniquely characterize p" - surely being C0 universal is not sufficient, as we also require e.g. the kernel to be differentiable?"}: 

Yes, the kernel must be at least twice continuously differentiable. We have now added this condition in the theorem.

\item {\it "as a non-expert, I was confused whether just before Theorem 3.4,
the basis being discussed is for the Lie group or the Lie algebra..."}: 

The basis being discussed here is for the Lie group. The vector field bases that we take are \textbf{left-invariant} vector fields, which is uniquely determined by its vector at the identity. Given two \textbf{left-invariant} vector bases $D^l$ and $E^k$, if their vectors at the identity $D^l_e$ and $E^k_e$ satisfy $D^l_e=\sum_{k} a^l_k E^k_e $, then the entire vector field will satisfy $D^l=\sum_{k} a^l_k E^k $.


\item {\it "I felt that the proof of Example 1 was not fully convincing..."}: 

If we consider the weighted term, then the equation in the proof will be
\[\vectz(F)^\top \cdot\sum_{i,j}A(X_i,X_j) \frac{q(X_i)}{w(X_i)}\frac{q(X_j)}{w(X_j)} \cdot \vectz(F)-2 \sum_{i,j} b(X_i,X_j) \frac{q(X_i)}{w(X_i)}\frac{q(X_j)}{w(X_j)} \cdot \vectz(F),  \]
then the result will be the one shown in the proof. We will clarify the confusions in the proof in the modified version.

\item{\it "but where did the authors assume the model was identifiable?"}: 

This assumption is not necessary in most of the results in this work. We have added this assumption to wherever it is needed, including theorem \ref{GoF} and the comment below theorem \ref{MKSDEconsistency}.


\item {\it "the rest of the proof is the same as the one given in [22] and [23]..."}: 

We have now modified the assumptions in theorem \ref{MKSDECLT} so as to be consistent with those in   \cite[Thm. 12]{oates2022minimum} and thus rest of the proof as stated is similar to that in \cite[Thm. 12]{oates2022minimum}.

\item {\it "(p9) what assumptions are being made on $V_{\theta_0}$ in Proposition 1?..."}: 

We have added the assumption on $V_{\theta_0}$ and a more precise reference.


\item {\it "Algorithm 2 looks strange to me because w appears to be independent of $\theta^t$..."}:

The weighted KSD $n^{-2}\sum k_\theta(x_i,x_j) q(x_i)q(x_j)w(x_i)^{-1}w(x_j)^{-1}$ involves a target distribution $q$ that we want to approximate, a candidate distribution family $\{p_\theta\}$ with which we will use to approximate $q$ and a easy-to-sample distribution $w$. The existence of $w$ is only to lower the difficulty of sampling, which is irrelevant to the approximation between $p_\theta$ and $q$. In $Q_{\wksd}(\theta|\theta^t)$, the distribution $p(z|\boldsymbol{x},\theta^t)$ plays the role of the target distribution $q$. We do not directly sample from $q$, instead we sample from $w$ and add a weighted ratio $q(x)/w(x)$.


\item {\it "In the "Characterization" theorem, where is the local Lipschitz property used? "} 

The local Lipschitz property is to make sure that the density $q$ is differentiable almost everywhere so that $D^l\log q$ exists. By the Rademacher's theorem, a locally Lipschitz function is differentiable everywhere. The assumption is not explicitly made in \cite{chwialkowski2016kernel}, but note that then theorem 2.2 in \cite{chwialkowski2016kernel} does require $\nabla\log q$ to exist.

\item {\it "the statement of Lemma 1 would be improved..."}

We have improved the statement of lemma 1. The statement of results in \cite{rubin1956uniform,yeo2001uniform} are rather long and clumsy, using symbols different from our work. We feel it would be better not to include them.
\end{enumerate}

\subsection{\bf Response to Reviewer-2}

Thank you for your valuable comments. We now address your major comments below. All suggested minor corrections have been incorporated into the body of the paper.

\subsubsection{\bf "Is the Stein operator new? What's the role of modular function?"} 

Yes, our Stein operator is novel, despite it being based on the divergence operator on manifolds. The divergence operator maps vector fields to scalar functions. However, the vector fields on Euclidean space can be regarded as vector-valued functions, so that for the divergence-type Stein operator on Euclidean space, one can consider the vector-valued RKHS as the Stein class. The divergence-type Stein operator on a manifold, e.g., \cite[\S 4.2.1]{barp2022geometric}, even though it maps vector fields to scalar functions, cannot be combined with a vector valued RKHS Stein class, since the vector fields on manifolds are not vector-valued functions. In this work, we use a basis of vector fields to establish a one-to-one correspondence between the vector fields and the vector-valued functions, so that the Stein class can be prescribed as RKHS, as we will elaborate next. The modular function is a necessary term in the operator.

The divergence-type Stein operator  is indeed the most commonly-adopted operator in both Euclidean space and non-flat manifolds. The main reason is the divergence theorem, with which one can easily construct the Stein operator and the Stein class that satisfy the Stein's identity. In Euclidean space $\mathbb{R}^d$, as introduced in our work, the Stein operator
\[
 T_p: f \mapsto \sum_{l=1}^d \left[\frac{\partial f_l}{\partial x^l} + f_l \frac{\partial}{\partial x^l} \log p\right] .
\]
is most commonly-adopted, which is a divergence-type Stein operator. It maps $f=(f_1,\dots,f_d)^\top$ to a real-valued function on $\mathbb{R}^d$. Note that $f$ is not only a vector-valued function so that the Stein class can be taken as a vector-valued RKHS, but also a vector field on $\mathbb{R}^d$ so that the divergence operator can act on it. However, the situation is different on manifold $M$. In \cite{barp2022geometric}, the authors define a divergence-type Stein operator $\mathrm{S}_\mu$ which maps vector fields $X$ in some Stein class $\mathscr{V}$ to functions on $M$. Since $X$ is not a multivariate function as in the Euclidean case, the Stein class $\mathscr{V}$ can not be taken as a vector-valued RKHS. \textit{To let a divergence-type Stein operator act on RKHS, the elements in the Stein class must be vector fields and vector-valued functions simultaneously}.

To combine the divergence-type Stein operator with the RKHS Stein class, one possible solution is to adopt the operator $T_p$ locally, since the manifold is locally Euclidean. In \cite{xu2021interpretable}, the authors defined the stein operator as:
\[
\mathcal{A}^{(1)}_p f:=\sum_{i=1}^d \left[\frac{\partial f^i}{\partial \theta^i}+ f^i\frac{\partial}{\partial \theta^i}\log(p J)\right],
\]
where $J$ is the volume element and $\theta^i$ are the local coordinates, see \cite[Eq. (5)]{xu2021interpretable}. However, note that the Stein operator $\mathcal{A}^{(1)}_p f= (p J)^{-1}\sum \frac{\partial}{\partial \theta^i}(f^i p J)$ clearly depends on the choice of the local chart $\theta^i$, \textit{thus by construction, $\mathcal{A}^{(1)}_p f$ is defined only within the chart 
%does not exceed the boundary of the local chart, 
and is not continuous on the boundary.} Therefore, the Stokes's theorem does not apply and thus the Stein identity does not hold. To tackle this issue, we must consider a partition of unity $\{\rho_\alpha\}$ subordinate to the atlas $\{(\theta_\alpha,U_\alpha)\}$, and define
\[
\mathcal{A}^{(1)}_p f:=\sum_\alpha\sum_{i=1}^d \left[\frac{\partial f^i\rho_\alpha }{\partial \theta_\alpha^i}+ f^i\rho_\alpha\frac{\partial}{\partial \theta^i}\log(p J)\right].
\]
However, such an operator will increase the difficulty of calculation enormously.

In contrast, our solution is to select a basis $X_i$, $1\leq i\leq d$ of the vector fields, i.e., for each vector field $X$ on $M$, there exists functions $f^i$, $1\leq i\leq d$ on $M$ such that $X=\sum_{i=1}^d f^i X_i $. We then define the Stein operator as
\[
\mathcal{A}_p f= p^{-1}\Div(p \sum_{i=1}^d f^i X_i )=\sum_{i=1}^d [X_i f^i+f^i X_i\log p+ f^i \Div X_i],
\]
where $f=(f^1,\dots,f^d)^\top$ and $X\log p$ represents the derivative of $\log p$ along $X$. Note that $\mathcal{A}_p f$ maps a vector-valued function, instead of a vector field, to a real-valued function, and thus the Stein class can be taken as a vector-valued RKHS. The decomposition $X=\sum_{i=1}^d f^i X_i $ establishes a one-to-one correspondence between the vector fields on $M$ and the vector-valued functions. 

The difficulty lies in the selection of $X_i$. Note that $X_i$ must form a basis of $T_x M$ at every point $x\in M$, so that it can decompose each vector field $X$ into $\sum_{i=1}^d f^i X_i$. In Euclidean case, we can let $X_i=\frac{\partial}{\partial x^i}$, and the the operator degenerates to $T_p$ since $\Div\frac{\partial}{\partial x^i}=0$. However, there is no general selection of $X_i$ on a general manifold. For example, by the hairy ball theorem \cite{Eisenberg1979}, there is no non-vanishing continuous tangent vector field on an even-dimensional n-sphere.
%every continuous vector field on an even-dimensional sphere must have a zero. 
Therefore, any $d$ vector fields $X_i$, $1\leq i\leq d$ on an even-dimensional sphere does not satisfy the requirements, since they all have a zero somewhere.

Despite the difficulty in this selection on general manifolds, the left-invariant basis $D^l$ is a natural choice of $X_i$ on Lie groups. \textit{The modular function term is exactly the divergence term $\Div X_i$ in the operator.} We can eliminate the modular function term by using the right-invariant vector fields. However, the modular functions of most Lie groups are readily available and thus it does not burden the calculation in practice. In addition, we want to be consistent in the choice of the left-invariance both on the vector fields and the Haar measure.

\subsubsection{\bf "Discussing other choices of kernels..."}  

To ensure that the KSD characterizes $p$ uniquely and that the MKSDE is convergent, we need the kernel function to satisfy the $C_0$-universality. On $\SO(N)$, we chose  $k(X,Y)=\exp(\tr(X^\top Y))$, which is a $C_0$-universal kernel function.  It is possible to construct other $C_0$-universal kernels, using for example the Laplace and the Mat\'{e}rn kernels in $\mathbb{R}^{N\times N}$ projected to $\SO(N)$. However, the derivation of closed forms for the MKSDE in these cases is rather complex and tedious but similar in spirit to what we have already illustrated for the chosen kernel. We have now stated this explicitly in the body of the revised paper. We will explore the practical advantages, if any, of these kernels in our future work.


\subsubsection{\bf "This is especially true for distributions of manifold-valued..."} 

What we are trying to convey here is that it is hard to compute the \textit{normalizing constant} of a distribution for a random variable that takes values in a non-flat space, as the symbolic integral calculation is generally intractable for most distributions on a non-flat space. A large fraction (percentage)  of the commonly used distribution families on $\mathbb{R}^d$ do have closed forms of their normalization constants. However, for many non-flat spaces, most of the commonly-used distribution families do not have closed forms for their normalizing constants, e.g., for the Bingham and von-Mises Fisher distributions on $\SO(N)$, it is a 
hypergeometric function of a matrix
argument and is a challenge to compute. This normalization factor and its gradient are most often approximated using numerical methods including table look ups that are cumbersome (see for e.g.,  \cite{Gilitschenski2019,Mohlin2020Neurips}).
%the von Mises-Fisher distribution and Kent distribution on the sphere $\mathbb{S}^{d-1}$, especially for $d > 3$. 

\subsubsection{\bf "... Stokes’s theorem does require..."} 

We are aware of the result you mentioned, see for example \cite[Thm. 17.30]{lee2013smooth} which states,
\begin{theorem*} Suppose $M$ is connected and oriented, then a compactly supported $d$-form $\omega$ is {\bf exact} iff $\int_M w =0$.
\end{theorem*}
The "only if" part is straightforward from the Stokes's theorem, and the "if" part is non-trivial and an application of the de Rham cohomology groups. However, it is noteworthy that such a result only applies to $d$-forms that are \textit{globally smooth}, and the authors of  \cite{xu2021interpretable} actually \textit{make use of the "only if" part of the theorem (the Stokes's theorem) instead of the converse}.
The authors defined the Stein operator as
\[
\mathcal{A}^{(1)}_p f:=\sum_{i=1}^d \left[\frac{\partial f^i}{\partial \theta^i}+ f^i\frac{\partial}{\partial \theta^i}\log(p J)\right],
\]
and show that $p\mathcal{A}^{(1)}_p f \Omega$ is an exact form so as to conclude that it integrates to $0$ by Stokes's theorem. Note that since the definition of $\mathcal{A}^{(1)}_p$ relies on the choice of local coordinates, it is \textit{not well-defined outside the chart.} To apply the Stokes's theorem in such a $d$-form, one must \textit{extend it smoothly to the entire manifold without violating the exactness condition stated in the above theorem}. This is highly non-trivial and possibly intractable.

\subsubsection{\bf Minor Comments}
 In this revision, we have fixed all typos and minor inaccuracies  that you had pointed out in our original submission. Your suggestions and comments requiring our explicit response and explanation are addressed in what follows:
 \begin{enumerate}[(a)]

\item {\it "On page 4: why is it ”clear” that..."}:

We have now included a more detailed explanation in this revised version, please see theorem \ref{KSDdiff}.

\item {\it "Concerning the line above Theorem 4.5..."}:

Although the Lie group structure does not play a role in the proof of theorem 4.5, this independence is not immediately obvious to everyone without the explicit presentation of the proof. In addition, the weighted term in the KSD plays a role in the proof.

\item{"Let $A_{ij}$ represent the...”: typo...}:

Yes it corresponds to $XE_{ij}$. We have fixed this typo in this revision.

\item {\it "Appendix page 12: what is div?..."} 

Yes, the divergence operator $\Div$ is with respect to the left-invariant Riemannian metric. As it is only used once in the appendix, we chose not to include it in the main text. We have now clarified the definition of $\Div$ in the proof of theorem \ref{KSDCharacterization}.
 \end{enumerate}





==> Rebuttals/SecondRebuttal.tex <==

\author{Xiaoda Qu, Xiran Fan, Baba C. Vemuri \thanks{Manuscript received February 2024}}
\begin{center}
{\Large \bf Kernel Stein Discrepancy on Lie Groups: Theory and Applications}
\end{center}

\begin{center}
{\large Xiaoda Qu, Xiran Fan, Baba C. Vemuri}
\end{center}
\vspace{5mm}

\section*{\bf\large Response to Reviewer-1}

\setcounter{page}{1}
\setcounter{subsection}{0}

We thank you for your valuable comments and suggestions for improving the clarity of our work. We have addressed all your questions in the following paragraphs. We hope you find our responses and revision satisfactory. The citations used in this response are in the bibliography of the revised submission.

\subsection{Sobolev-type kernels}

 We have modified our description of the work by Barp et al. \cite{barp2018riemann} to read as follows: "In \cite{barp2018riemann}, Barp et al. adopted a second order Stein's operator free from the choice of coordinate charts in constructing an approximation to the posterior expectation of distributions supported only on compact manifolds. In addition, to successfully characterizing \(p\) uniquely with the KSD corresponding to this operator, one must consider a very large RKHS, i.e., the Sobolev space on $M$. Finding such a Sobolev space with an easy-to-derive closed form kernel can be challenging on a highly curved manifold. A possible way to address this challenge is to use the restriction of a Sobolev-type kernel on $\mathbb{R}^d$ to the manifold \cite{fuselier2012scattered}. "

There is however an unresolved issue at this juncture i.e., it is not obvious to us if the "algebraic Fourier decay" condition on the kernels in \cite{fuselier2012scattered} is flexible (lax) enough for us to find an easy-to-derive closed-form kernel. %To the best of our knowledge, 
The Matérn kernels used in \cite{fuselier2012scattered} (contain a modified Bessel function), as well as the original kernel function (in integral form) of Sobolev space on $\mathbb{R}^d$ in \cite{novak2018reproducing}, satisfy this condition but are not in a closed form and hence not easy-to-use in our setting. To the best of our knowledge, whether other kernels restricted to complete compact manifolds that satisfy the algebraic Fourier decay yield closed form expressions is an  open research problem. This however is beyond the scope of our work in here but will be the focus of our future research.

%We feel that this is an interesting open research problem that is beyond the scope of this paper but we will address in the near future. %We highly welcome if you can enlighten us with any feasible example, as this will also benefit our future research.

\subsection{Github codes}
We apologize for the error in the permissions on the URL. The link has been fixed now and is accessible at:  \url{https://github.com/cvgmi/KSD-on-Lie-Groups}.

\subsection{Central limit theorem}

We apologize for the inadvertent
mismatch between the conditions in theorem \ref{MKSDECLT} and \cite[Thm. 12]{oates2022minimum}. We have now fixed the conditions to match perfectly.
